Efficient and Robust Continual Graph Learning for Graph Classification in Biology

Graph classification is essential for understanding complex biological systems, where molecular structures and interactions are naturally represented as graphs. Traditional graph neural networks (GNNs) perform well on static tasks but struggle in dynamic settings due to catastrophic forgetting. We present Perturbed and Sparsified Continual Graph Learning (PSCGL), a robust and efficient continual graph learning framework for graph data classification, specifically targeting biological datasets. We introduce a perturbed sampling strategy to identify critical data points that contribute to model learning and a motif-based graph sparsification technique to reduce storage needs while maintaining performance. Additionally, our PSCGL framework inherently defends against graph backdoor attacks, which is crucial for applications in sensitive biological contexts. Extensive experiments on biological datasets demonstrate that PSCGL not only retains knowledge across tasks but also enhances the efficiency and robustness of graph classification models in biology.

==> Sections/Preliminary.tex <==
\section{Preliminaries}
\subsection{Notations}
Assume that the model receives a sequence of disjoint tasks $\mathcal{T} = \{\mathcal{T}_1, \mathcal{T}_2, \cdots, \mathcal{T}_K$\}. For each task $\mathcal{T}_t$, there is a corresponding dataset $D_t$ that is consisted of i.i.d graph data points $x_i = \{(X_{i}^{t}, A_{i}^{t}, y_{i}^{t})_{i=1}^{|D_t|}\}$. $X_{i}^{t} \in \mathcal{X} = \mathbb{R}^{T \times D}$ is the node feature matrix and $A_{i}^{t} \in \mathcal{A} = \{0, 1\}^{D \times D}$ is the adjacency matrix of the $i^{th}$ sample in the dataset $D_t$ corresponding to the task $\mathcal{T}_t$, and $y_{i}^{t} \in \mathcal{Y}^{t}$ is the corresponding ground truth label, where $\mathcal{Y}^{t}$ is the label space of task $\gT_t$. We assume that each task $\gT_t$ contains a set of unique class labels, where $\mathcal{Y}^{t} \cap \mathcal{Y}^{t'} = \emptyset$ for $t \neq t'$. Let the graph classifier $f$ be parameterized by $\theta$, and let $\ell$ be the cross-entropy loss function for classification loss. Additionally, the latent embedding of $x_i$ generated by $f$ is denoted as $h_i$. We denote $\mathcal{B}$ as the memory buffer with a budget $b$ for each class, and $\mathcal{L}_{\mathcal{B}}$ denotes the memory replay loss over the entire buffer. We use $\Phi$ to represent the perturbation functions used on the node feature matrix. 

\subsection{Graph-level Continual Graph Learning}

The general Continual Graph Learning (CGL) can be categorized into node-level and graph level settings \cite{zhang_cglb_2022}. We focus on graph-level continual graph learning (G-CGL) in this paper. The G-CGL shares similar characteristics with the traditional continual learning, where the entire graph is considered as one sample input. 

\subsection{Memory-Replay based methods}
Picking Anchor points after perturbation
